GRACES observations of young [alpha/Fe]-rich stars

We measure chemical abundance ratios and radial velocities in four massive (i.e., young) [alpha/Fe]-rich red giant stars using high-resolution high-S/N spectra from ESPaDOnS fed by Gemini-GRACES. Our differential analysis ensures that our chemical abundances are on the same scale as the Alves-Brito et al. (2010) study of bulge, thin and thick disk red giants. We confirm that the program stars have enhanced [alpha/Fe] ratios and are slightly metal poor. Aside from lithium enrichment in one object, the program stars exhibit no chemical abundance anomalies when compared to giant stars of similar metallicity throughout the Galaxy. This includes the elements Li, O, Si, Ca, Ti, Cr, Ni, Cu, Ba, La, and Eu. Therefore, there are no obvious chemical signatures that can help to reveal the origin of these unusual stars. While our new observations show that only one star (not the Li-rich object) exhibits a radial velocity variation, simulations indicate that we cannot exclude the possibility that all four could be binaries. In addition, we find that two (possibly three) stars show evidence for an infrared excess, indicative of a debris disk. This is consistent with these young [alpha/Fe]-rich stars being evolved blue stragglers, suggesting their apparent young age is a consequence of a merger or mass transfer. We would expect a binary fraction of ~50% or greater for the entire sample of these stars, but the signs of the circumbinary disk may have been lost since these features can have short timescales. Radial velocity monitoring is needed to confirm the blue straggler origin.

==> tab3.tex <==
\begin{table*}
 \centering
 \begin{minipage}{180mm}
  \caption{Line list for the program stars\label{tab:ew}}
  \begin{tabular}{@{}cccrrrrrrrrrrrrrrrc@{}}
  \hline
Wavelength & 
Species\footnote{The digits to the left of the decimal point are the atomic
number. The digit to the right of the decimal point is the ionization state
(``0'' = neutral, ``1'' = singly ionised).} & 
L.E.P & 
$\log gf$ & 
KIC 4350501 &
KIC 9821622 & 
KIC 11394905 & 
KIC 4143460 & 
HD 40409 & 
Source\footnote{A = $\log gf$ values used in \citet{Yong:2005aa} where the
references include \citet{Ivans:2001aa}, \citet{Kurucz:1995aa},
\citet{Prochaska:2000ab}, \citet{Ramirez:2002aa}; 
B = \citet{Gratton:2003aa};
C = Oxford group including 
\citet{Blackwell:1979aa,Blackwell:1979ab,Blackwell:1980aa,Blackwell:1986aa,Blackwell:1995aa}; 
D = \citet{Fuhr:2006aa}, using line component patterns for 
     hfs/IS from \citet{Kurucz:1995aa}; 
E = \citet{Fuhr:2006aa}, using hfs/IS from \citet{McWilliam:1998aa};
F = \citet{Lawler:2001aa}, using hfs from \citet{Ivans:2006aa};
G = \citet{Lawler:2001ab}, using hfs/IS from \citet{Ivans:2006aa}.  
\\
~
\\ 
This table is published in its entirety in the electronic edition of the paper.
A portion is shown here for guidance regarding its form and content.} \\ 
\AA & 
 & 
eV & 
 & 
m\AA & 
m\AA & 
m\AA & 
m\AA & 
m\AA & 
 \\ 
(1) & 
(2) &
(3) &
(4) & 
(5) & 
(6) & 
(7) & 
(8) & 
(9) & 
(10) \\ 
\hline
 6300.31 &    8.0 &   0.00 & $-$9.75 &   \multicolumn{5}{c}{Spectrum synthesis}             &           B \\
 7771.95 &    8.0 &   9.15 &    0.35 &     38.5 &     39.2 &   \ldots &     45.6 &     29.4 &           B \\
 7774.18 &    8.0 &   9.15 &    0.21 &     38.0 &     30.6 &     39.3 &     43.6 &     33.9 &           B \\
 5665.56 &   14.0 &   4.92 & $-$2.04 &     56.0 &     48.7 &     46.3 &     57.4 &     67.5 &           B \\
 5684.49 &   14.0 &   4.95 & $-$1.65 &     69.2 &   \ldots &   \ldots &   \ldots &   \ldots &           B \\
 5690.43 &   14.0 &   4.93 & $-$1.87 &     61.1 &     54.5 &     53.8 &     60.7 &     62.1 &           B \\
 5701.11 &   14.0 &   4.93 & $-$2.05 &     49.5 &     45.3 &     43.9 &     49.4 &     53.0 &           B \\
 5772.15 &   14.0 &   5.08 & $-$1.75 &     65.8 &   \ldots &   \ldots &   \ldots &   \ldots &           B \\
 5793.08 &   14.0 &   4.93 & $-$2.06 &     56.7 &     49.6 &     50.5 &     59.7 &     61.2 &           B \\
 5948.55 &   14.0 &   5.08 & $-$1.23 &     90.0 &     85.2 &     90.7 &     94.7 &    101.1 &           B \\
 6125.03 &   14.0 &   5.62 & $-$1.57 &     38.0 &     36.1 &     32.5 &     42.6 &   \ldots &           B \\
 6142.49 &   14.0 &   5.62 & $-$1.43 &     40.1 &     34.9 &     33.8 &     39.0 &     41.4 &           B \\
 6145.02 &   14.0 &   5.62 & $-$1.49 &     40.9 &     39.8 &     37.5 &     45.9 &     46.7 &           B \\
 6155.14 &   14.0 &   5.62 & $-$0.86 &     79.0 &     73.5 &     72.2 &     80.0 &   \ldots &           B \\
 6237.33 &   14.0 &   5.62 & $-$1.08 &     65.0 &     56.6 &     56.1 &     66.6 &   \ldots &           B \\
 6244.48 &   14.0 &   5.62 & $-$1.29 &     51.1 &     47.6 &     46.2 &   \ldots &   \ldots &           B \\
 6414.99 &   14.0 &   5.87 & $-$1.03 &   \ldots &     43.2 &   \ldots &   \ldots &   \ldots &           B \\
 6721.84 &   14.0 &   5.86 & $-$1.16 &     51.1 &     44.7 &     40.1 &     51.8 &     61.5 &           B \\
 6848.57 &   14.0 &   5.86 & $-$1.75 &     25.8 &     22.1 &   \ldots &   \ldots &     28.6 &           B \\
 7405.79 &   14.0 &   5.62 & $-$0.82 &     95.5 &     82.9 &     90.2 &     92.7 &     99.3 &           B \\
 5260.39 &   20.0 &   2.52 & $-$1.72 &     55.0 &     55.8 &     40.6 &     57.0 &     71.2 &           B \\
 5261.71 &   20.0 &   2.52 & $-$0.58 &    118.0 &    116.7 &    111.0 &    122.3 &   \ldots &           B \\
 5512.99 &   20.0 &   2.93 & $-$0.45 &     99.8 &   \ldots &     91.0 &    101.2 &   \ldots &           A \\
 5581.98 &   20.0 &   2.52 & $-$0.56 &    114.2 &    110.8 &    101.0 &    110.8 &   \ldots &           A \\
 5590.13 &   20.0 &   2.51 & $-$0.57 &    107.2 &    104.0 &    101.1 &    111.5 &   \ldots &           B \\
 5867.57 &   20.0 &   2.93 & $-$1.49 &     48.5 &     44.7 &     31.9 &     47.1 &     61.8 &           B \\
 6166.44 &   20.0 &   2.52 & $-$1.14 &     97.3 &     93.0 &     83.3 &     98.0 &    113.1 &           B \\
 6169.04 &   20.0 &   2.52 & $-$0.80 &   \ldots &    110.5 &    100.1 &    117.7 &   \ldots &           B \\
 6169.56 &   20.0 &   2.52 & $-$0.48 &   \ldots &    122.5 &   \ldots &   \ldots &   \ldots &           B \\
 6471.67 &   20.0 &   2.52 & $-$0.69 &    119.5 &    117.5 &   \ldots &    121.7 &   \ldots &           B \\
 6499.65 &   20.0 &   2.52 & $-$0.82 &    115.5 &    110.5 &    100.5 &    116.6 &   \ldots &           B \\
 5016.17 &   22.0 &   0.85 & $-$0.57 &   \ldots &    109.6 &    103.8 &    115.2 &   \ldots &           B \\
 5022.87 &   22.0 &   0.83 & $-$0.43 &   \ldots &    120.3 &    106.4 &   \ldots &   \ldots &           B \\
 5039.96 &   22.0 &   0.02 & $-$1.13 &   \ldots &    122.7 &    116.5 &   \ldots &   \ldots &           B \\
 5043.59 &   22.0 &   0.84 & $-$1.73 &   \ldots &     68.2 &     48.7 &     66.1 &   \ldots &           B \\
 5145.47 &   22.0 &   1.46 & $-$0.57 &   \ldots &     81.2 &   \ldots &   \ldots &   \ldots &           B \\
 5147.48 &   22.0 &   0.00 & $-$2.01 &   \ldots &     99.3 &   \ldots &   \ldots &   \ldots &           B \\
 5219.71 &   22.0 &   0.02 & $-$2.29 &   \ldots &   \ldots &   \ldots &     92.8 &    108.5 &           B \\
 5223.63 &   22.0 &   2.09 & $-$0.56 &     50.9 &     47.0 &     34.5 &     49.3 &     70.1 &           B \\
 5295.78 &   22.0 &   1.05 & $-$1.63 &     62.3 &     56.5 &     42.5 &     57.6 &     70.6 &           B \\
 5299.98 &   22.0 &   1.05 & $-$1.36 &     42.9 &   \ldots &     22.6 &   \ldots &     62.7 &           B \\
 5490.16 &   22.0 &   1.46 & $-$0.93 &     67.5 &     65.8 &   \ldots &   \ldots &   \ldots &           B \\
 5648.57 &   22.0 &   2.49 & $-$0.25 &     42.9 &     35.7 &     25.1 &     39.2 &     52.2 &           A \\
 5679.94 &   22.0 &   2.47 & $-$0.58 &     31.1 &     23.7 &   \ldots &   \ldots &   \ldots &           A \\
 5689.48 &   22.0 &   2.30 & $-$0.47 &     47.5 &     42.8 &     29.5 &     46.1 &     61.4 &           B \\
 5702.69 &   22.0 &   2.29 & $-$0.57 &     32.8 &     31.2 &   \ldots &     32.2 &   \ldots &           A \\
 5716.46 &   22.0 &   2.30 & $-$0.70 &     33.0 &     25.5 &   \ldots &     26.8 &     44.0 &           A \\
 5739.46 &   22.0 &   2.25 & $-$0.60 &     38.5 &   \ldots &     20.1 &     32.5 &     48.7 &           A \\
 5739.98 &   22.0 &   2.24 & $-$0.67 &     26.6 &     24.5 &   \ldots &     26.2 &     40.2 &           A \\
 5866.46 &   22.0 &   1.07 & $-$0.84 &    104.2 &    100.2 &     89.9 &    110.0 &   \ldots &           B \\
 5880.27 &   22.0 &   1.05 & $-$2.05 &     44.8 &     41.8 &     28.3 &   \ldots &   \ldots &           A \\
 5903.32 &   22.0 &   1.07 & $-$2.14 &     46.4 &     34.5 &     20.2 &     36.5 &     57.7 &           A \\
 5922.12 &   22.0 &   1.05 & $-$1.47 &     74.2 &     74.5 &   \ldots &   \ldots &   \ldots &           B \\
 5937.81 &   22.0 &   1.07 & $-$1.89 &     49.0 &     43.1 &     28.9 &     47.7 &     65.7 &           A \\
 5941.75 &   22.0 &   1.05 & $-$1.52 &     71.3 &     72.7 &     56.0 &     70.3 &   \ldots &           A \\
 5999.68 &   22.0 &   2.17 & $-$0.73 &     33.2 &     29.4 &     18.8 &     33.2 &     44.0 &           A \\
 6091.18 &   22.0 &   2.27 & $-$0.42 &     59.4 &     48.5 &     36.9 &     52.5 &     66.9 &           B \\
 6126.22 &   22.0 &   1.07 & $-$1.42 &     79.8 &     76.2 &     60.4 &     80.8 &     94.0 &           B \\
 6146.22 &   22.0 &   1.87 & $-$1.47 &     22.8 &     19.9 &   \ldots &   \ldots &   \ldots &           A \\
 6186.15 &   22.0 &   2.17 & $-$1.15 &     30.9 &   \ldots &   \ldots &     26.6 &     49.2 &           A \\
 6258.11 &   22.0 &   1.44 & $-$0.36 &   \ldots &     98.8 &     91.0 &   \ldots &   \ldots &           B \\
 6303.76 &   22.0 &   1.44 & $-$1.57 &   \ldots &     44.5 &   \ldots &     46.5 &   \ldots &           A \\
 6312.24 &   22.0 &   1.46 & $-$1.55 &     50.0 &     42.4 &   \ldots &     45.6 &     59.4 &           A \\
 6497.69 &   22.0 &   1.44 & $-$1.93 &   \ldots &     26.8 &   \ldots &   \ldots &     43.9 &           A \\
 6508.14 &   22.0 &   1.43 & $-$1.98 &     24.4 &     19.5 &   \ldots &   \ldots &     41.4 &           A \\
 6554.24 &   22.0 &   1.44 & $-$1.22 &   \ldots &     63.3 &   \ldots &     66.0 &   \ldots &           B \\
 6716.68 &   22.0 &   2.49 & $-$1.04 &     12.8 &     10.8 &      6.9 &     10.7 &     19.0 &           A \\
 6743.12 &   22.0 &   0.90 & $-$1.63 &     80.5 &     75.8 &     56.4 &   \ldots &    103.5 &           A \\
 5214.13 &   24.0 &   3.37 & $-$0.74 &   \ldots &   \ldots &   \ldots &   \ldots &     47.6 &           B \\
 5238.97 &   24.0 &   2.71 & $-$1.30 &     34.1 &     29.0 &   \ldots &     32.2 &     54.3 &           B \\
 5300.75 &   24.0 &   0.98 & $-$2.13 &     97.8 &     92.5 &     85.0 &     99.6 &   \ldots &           B \\
 5304.19 &   24.0 &   3.46 & $-$0.69 &     28.6 &   \ldots &   \ldots &   \ldots &   \ldots &           B \\
 5312.86 &   24.0 &   3.45 & $-$0.56 &   \ldots &     26.9 &   \ldots &   \ldots &   \ldots &           B \\
 5318.78 &   24.0 &   3.44 & $-$0.69 &   \ldots &   \ldots &     16.1 &   \ldots &   \ldots &           B \\
 5348.33 &   24.0 &   1.00 & $-$1.29 &   \ldots &   \ldots &    123.5 &   \ldots &   \ldots &           B \\
 5628.65 &   24.0 &   3.42 & $-$0.77 &     28.2 &     21.1 &     14.8 &   \ldots &   \ldots &           B \\
 5702.33 &   24.0 &   3.45 & $-$0.68 &     48.6 &     39.7 &     35.4 &     47.5 &     73.1 &           B \\
 5783.07 &   24.0 &   3.32 & $-$0.40 &   \ldots &   \ldots &   \ldots &     49.0 &     72.1 &           B \\
 5783.87 &   24.0 &   3.32 & $-$0.30 &     74.5 &   \ldots &   \ldots &   \ldots &     98.0 &           B \\
 5787.93 &   24.0 &   3.32 & $-$0.08 &     63.5 &     60.2 &     51.8 &     64.5 &     85.7 &           B \\
 6883.07 &   24.0 &   3.44 & $-$0.42 &     56.1 &     42.8 &     30.5 &     48.5 &   \ldots &           B \\
 5016.48 &   26.0 &   4.26 & $-$1.62 &   \ldots &     39.6 &   \ldots &     43.2 &   \ldots &           B \\
 5044.21 &   26.0 &   2.85 & $-$2.03 &   \ldots &     96.8 &     90.5 &   \ldots &   \ldots &           C \\
 5054.64 &   26.0 &   3.64 & $-$1.94 &   \ldots &     51.2 &     47.0 &     54.0 &   \ldots &           C \\
 5058.49 &   26.0 &   3.64 & $-$2.76 &     23.2 &   \ldots &   \ldots &   \ldots &   \ldots &           B \\
 5060.08 &   26.0 &   0.00 & $-$5.45 &   \ldots &   \ldots &    106.6 &   \ldots &   \ldots &           C \\
 5187.92 &   26.0 &   4.14 & $-$1.27 &   \ldots &     69.5 &     63.5 &     75.8 &   \ldots &           B \\
 5196.06 &   26.0 &   4.26 & $-$0.87 &   \ldots &     79.5 &     73.0 &     80.7 &   \ldots &           B \\
 5198.72 &   26.0 &   2.22 & $-$2.14 &    122.8 &   \ldots &    115.2 &   \ldots &   \ldots &           B \\
 5223.19 &   26.0 &   3.64 & $-$2.28 &     47.6 &   \ldots &     35.5 &   \ldots &     60.7 &           B \\
 5225.53 &   26.0 &   0.11 & $-$4.79 &    119.8 &    119.8 &    119.5 &   \ldots &   \ldots &           B \\
 5242.49 &   26.0 &   3.63 & $-$0.98 &     97.1 &     94.8 &     94.8 &    103.3 &    112.9 &           C \\
 5243.78 &   26.0 &   4.26 & $-$1.01 &     70.2 &     68.2 &     64.0 &     74.5 &     88.2 &           B \\
 5250.22 &   26.0 &   0.12 & $-$4.94 &   \ldots &   \ldots &    114.6 &   \ldots &   \ldots &           B \\
 5253.03 &   26.0 &   2.28 & $-$3.84 &     48.7 &     44.2 &     36.8 &     51.5 &   \ldots &           B \\
 5253.46 &   26.0 &   3.28 & $-$1.63 &   \ldots &     88.5 &     87.2 &   \ldots &   \ldots &           C \\
 5288.53 &   26.0 &   3.69 & $-$1.53 &   \ldots &     69.1 &     69.8 &   \ldots &   \ldots &           C \\
 5294.55 &   26.0 &   3.64 & $-$2.70 &     33.7 &     26.8 &   \ldots &   \ldots &   \ldots &           B \\
 5295.32 &   26.0 &   4.42 & $-$1.55 &   \ldots &     36.1 &     32.4 &     41.1 &     51.0 &           B \\
 5321.11 &   26.0 &   4.44 & $-$1.23 &     52.3 &     46.8 &     41.9 &   \ldots &     65.0 &           B \\
 5326.14 &   26.0 &   3.57 & $-$2.13 &     59.2 &     54.0 &     46.0 &     57.5 &   \ldots &           C \\
 5326.82 &   26.0 &   4.42 & $-$2.09 &     23.7 &   \ldots &   \ldots &   \ldots &   \ldots &           B \\
 5367.48 &   26.0 &   4.41 &    0.43 &   \ldots &   \ldots &   \ldots &    120.0 &   \ldots &           C \\
 5379.58 &   26.0 &   3.70 & $-$1.43 &     79.9 &     69.7 &     70.7 &     78.5 &     91.5 &           B \\
 5386.34 &   26.0 &   4.16 & $-$1.74 &     46.2 &     42.1 &     34.4 &     46.6 &     60.5 &           B \\
 5389.49 &   26.0 &   4.42 & $-$0.52 &     87.3 &     84.2 &     85.8 &     88.4 &   \ldots &           B \\
 5395.22 &   26.0 &   4.45 & $-$1.73 &     35.2 &     25.8 &     21.9 &     30.1 &   \ldots &           B \\
 5398.29 &   26.0 &   4.45 & $-$0.68 &     81.7 &     75.8 &     75.7 &     82.3 &   \ldots &           B \\
 5401.27 &   26.0 &   4.32 & $-$1.74 &   \ldots &   \ldots &     34.2 &   \ldots &   \ldots &           B \\
 5406.78 &   26.0 &   4.37 & $-$1.39 &     52.9 &     42.5 &     38.6 &     47.8 &   \ldots &           B \\
 5412.79 &   26.0 &   4.44 & $-$1.72 &   \ldots &   \ldots &     22.8 &   \ldots &   \ldots &           B \\
 5417.04 &   26.0 &   4.42 & $-$1.42 &     51.4 &     39.2 &     39.0 &     44.6 &     61.9 &           B \\
 5464.29 &   26.0 &   4.14 & $-$1.62 &   \ldots &     45.9 &     44.0 &   \ldots &   \ldots &           B \\
 5470.09 &   26.0 &   4.45 & $-$1.60 &   \ldots &     32.3 &     23.1 &   \ldots &     53.3 &           B \\
 5491.84 &   26.0 &   4.18 & $-$2.25 &     21.1 &     16.9 &     14.8 &   \ldots &   \ldots &           C \\
 5494.47 &   26.0 &   4.08 & $-$1.96 &     45.8 &   \ldots &   \ldots &   \ldots &   \ldots &           B \\
 5522.45 &   26.0 &   4.21 & $-$1.45 &     59.4 &     49.5 &     43.6 &     55.9 &     69.7 &           B \\
 5525.54 &   26.0 &   4.23 & $-$1.15 &     66.8 &     63.2 &     59.4 &     68.5 &   \ldots &           C \\
 5539.29 &   26.0 &   3.64 & $-$2.59 &     35.4 &   \ldots &     26.0 &     34.5 &   \ldots &           B \\
 5560.22 &   26.0 &   4.44 & $-$1.07 &     60.4 &     53.4 &     54.0 &     59.2 &     73.9 &           B \\
 5587.58 &   26.0 &   4.14 & $-$1.70 &   \ldots &     46.0 &   \ldots &   \ldots &   \ldots &           B \\
 5618.64 &   26.0 &   4.21 & $-$1.32 &     59.5 &   \ldots &   \ldots &   \ldots &   \ldots &           B \\
 5619.61 &   26.0 &   4.39 & $-$1.49 &   \ldots &     41.9 &   \ldots &   \ldots &   \ldots &           B \\
 5635.83 &   26.0 &   4.26 & $-$1.59 &     55.0 &     42.5 &   \ldots &     49.3 &   \ldots &           B \\
 5651.48 &   26.0 &   4.47 & $-$1.79 &     28.6 &     24.2 &     19.7 &     26.1 &   \ldots &           B \\
 5652.33 &   26.0 &   4.26 & $-$1.77 &     41.0 &   \ldots &   \ldots &     40.3 &   \ldots &           B \\
 5661.35 &   26.0 &   4.29 & $-$1.76 &     43.0 &     33.6 &     26.5 &     36.9 &   \ldots &           B \\
 5662.51 &   26.0 &   4.18 & $-$0.59 &   \ldots &   \ldots &     96.0 &    102.4 &   \ldots &           C \\
 5701.56 &   26.0 &   2.56 & $-$2.22 &   \ldots &    105.0 &   \ldots &    115.0 &   \ldots &           B \\
 5705.47 &   26.0 &   4.30 & $-$1.42 &     51.9 &     45.5 &     40.4 &     53.4 &     67.8 &           C \\
 5717.84 &   26.0 &   4.29 & $-$0.94 &   \ldots &   \ldots &     66.7 &   \ldots &   \ldots &           B \\
 5731.77 &   26.0 &   4.26 & $-$1.08 &     68.5 &     61.9 &     62.2 &     70.8 &     88.3 &           B \\
 5738.24 &   26.0 &   4.22 & $-$2.24 &     22.1 &   \ldots &     14.0 &   \ldots &     40.6 &           B \\
 5752.04 &   26.0 &   4.55 & $-$0.96 &     64.4 &   \ldots &   \ldots &   \ldots &     76.6 &           B \\
 5760.36 &   26.0 &   3.64 & $-$2.46 &     41.2 &   \ldots &   \ldots &   \ldots &   \ldots &           B \\
 5778.46 &   26.0 &   2.59 & $-$3.44 &     53.3 &     47.6 &     41.0 &     54.5 &     68.3 &           B \\
 5793.92 &   26.0 &   4.22 & $-$1.62 &     51.7 &     41.5 &   \ldots &   \ldots &     64.7 &           B \\
 5806.73 &   26.0 &   4.61 & $-$0.91 &     67.7 &     57.8 &     56.5 &   \ldots &     84.1 &           B \\
 5814.81 &   26.0 &   4.28 & $-$1.81 &     39.4 &     32.8 &     24.7 &     37.5 &     51.2 &           B \\
 5835.11 &   26.0 &   4.26 & $-$2.18 &   \ldots &     20.2 &   \ldots &   \ldots &   \ldots &           B \\
 5852.23 &   26.0 &   4.55 & $-$1.17 &     58.6 &   \ldots &     43.5 &     56.4 &     82.8 &           B \\
 5855.09 &   26.0 &   4.61 & $-$1.48 &     31.9 &     25.8 &     21.4 &     29.7 &     45.6 &           B \\
 5858.78 &   26.0 &   4.22 & $-$2.19 &     24.1 &     18.2 &   \ldots &   \ldots &     38.1 &           B \\
 5862.37 &   26.0 &   4.55 & $-$0.50 &     91.0 &     85.9 &     79.8 &     91.5 &   \ldots &           B \\
 5902.48 &   26.0 &   4.59 & $-$1.86 &     22.1 &     16.8 &     13.4 &     18.4 &     33.5 &           B \\
 5905.68 &   26.0 &   4.65 & $-$0.76 &     68.3 &     60.1 &     57.2 &     67.0 &     83.5 &           B \\
 5909.97 &   26.0 &   3.21 & $-$2.64 &     61.3 &     53.5 &     53.5 &     65.9 &   \ldots &           C \\
 5916.25 &   26.0 &   2.45 & $-$2.99 &     83.8 &   \ldots &   \ldots &   \ldots &   \ldots &           C \\
 5929.68 &   26.0 &   4.55 & $-$1.24 &     53.8 &     46.9 &     44.0 &     51.5 &   \ldots &           B \\
 5930.19 &   26.0 &   4.65 & $-$0.29 &     95.5 &     83.5 &     86.5 &     95.7 &   \ldots &           B \\
 5934.67 &   26.0 &   3.93 & $-$1.15 &     90.4 &     80.7 &   \ldots &     92.2 &   \ldots &           B \\
 5956.71 &   26.0 &   0.86 & $-$4.60 &     97.7 &   \ldots &   \ldots &   \ldots &   \ldots &           B \\
 5976.79 &   26.0 &   3.94 & $-$1.33 &     82.2 &   \ldots &   \ldots &     86.5 &     97.7 &           B \\
 6003.02 &   26.0 &   3.88 & $-$1.08 &     90.8 &     87.5 &     86.8 &     93.3 &   \ldots &           B \\
 6008.57 &   26.0 &   3.88 & $-$0.96 &   \ldots &   \ldots &     90.8 &     96.8 &   \ldots &           B \\
 6012.21 &   26.0 &   2.22 & $-$4.07 &     53.7 &   \ldots &     38.8 &     53.8 &     74.8 &           C \\
 6027.06 &   26.0 &   4.08 & $-$1.23 &     76.2 &     72.5 &     71.5 &     80.9 &   \ldots &           B \\
 6056.01 &   26.0 &   4.73 & $-$0.42 &     80.8 &     85.6 &   \ldots &   \ldots &   \ldots &           B \\
 6079.02 &   26.0 &   4.65 & $-$0.95 &     57.5 &     52.2 &     48.1 &     58.5 &     70.8 &           B \\
 6089.57 &   26.0 &   4.58 & $-$1.28 &     56.8 &     45.9 &     44.8 &     56.0 &     68.8 &           B \\
 6093.65 &   26.0 &   4.61 & $-$1.32 &     41.4 &     34.5 &     31.3 &     40.3 &     56.4 &           B \\
 6094.38 &   26.0 &   4.65 & $-$1.56 &     30.8 &     24.2 &     19.6 &     26.9 &     44.0 &           B \\
 6096.67 &   26.0 &   3.98 & $-$1.77 &     58.1 &     47.2 &     44.6 &     52.9 &     69.7 &           B \\
 6098.25 &   26.0 &   4.56 & $-$1.81 &     28.1 &     21.2 &   \ldots &   \ldots &   \ldots &           B \\
 6120.24 &   26.0 &   0.91 & $-$5.97 &     32.5 &     28.8 &     18.2 &     31.8 &     50.0 &           C \\
 6151.62 &   26.0 &   2.18 & $-$3.30 &     84.5 &     76.8 &     76.3 &     86.0 &     98.4 &           B \\
 6165.36 &   26.0 &   4.14 & $-$1.50 &     62.0 &     53.9 &     48.3 &     59.4 &     75.2 &           B \\
 6173.34 &   26.0 &   2.22 & $-$2.88 &     97.4 &     93.3 &     93.7 &   \ldots &   \ldots &           B \\
 6200.32 &   26.0 &   2.61 & $-$2.44 &    100.6 &     92.5 &     95.7 &    102.5 &   \ldots &           B \\
 6213.44 &   26.0 &   2.22 & $-$2.54 &    108.7 &    105.7 &    107.5 &    116.0 &   \ldots &           B \\
 6226.74 &   26.0 &   3.88 & $-$2.08 &     48.8 &     40.0 &     34.0 &     44.1 &     62.2 &           B \\
 6229.23 &   26.0 &   2.84 & $-$2.85 &   \ldots &   \ldots &   \ldots &     69.7 &   \ldots &           C \\
 6232.65 &   26.0 &   3.65 & $-$1.22 &   \ldots &     91.1 &     90.5 &    101.2 &   \ldots &           B \\
 6240.65 &   26.0 &   2.22 & $-$3.23 &     82.5 &     77.3 &     73.2 &     86.5 &   \ldots &           B \\
 6246.33 &   26.0 &   3.60 & $-$0.73 &   \ldots &   \ldots &    113.0 &    122.3 &   \ldots &           B \\
 6265.14 &   26.0 &   2.18 & $-$2.55 &    123.3 &   \ldots &    114.7 &   \ldots &   \ldots &           B \\
 6270.23 &   26.0 &   2.86 & $-$2.46 &     80.5 &     71.0 &     72.6 &     81.2 &   \ldots &           B \\
 6271.28 &   26.0 &   3.33 & $-$2.76 &   \ldots &   \ldots &     34.4 &   \ldots &   \ldots &           C \\
 6301.51 &   26.0 &   3.65 & $-$0.72 &   \ldots &   \ldots &    112.5 &   \ldots &   \ldots &           B \\
 6315.81 &   26.0 &   4.08 & $-$1.68 &     61.2 &   \ldots &     57.1 &     61.1 &     74.5 &           B \\
 6322.69 &   26.0 &   2.59 & $-$2.43 &    101.2 &    100.2 &     94.3 &    108.8 &    124.2 &           B \\
 6330.85 &   26.0 &   4.73 & $-$1.22 &     46.0 &     38.1 &     31.6 &     41.4 &     56.9 &           B \\
 6335.34 &   26.0 &   2.20 & $-$2.27 &   \ldots &    121.5 &    124.0 &   \ldots &   \ldots &           B \\
 6336.82 &   26.0 &   3.68 & $-$0.92 &   \ldots &   \ldots &    103.5 &    112.3 &   \ldots &           C \\
 6380.75 &   26.0 &   4.19 & $-$1.37 &     71.5 &   \ldots &   \ldots &   \ldots &   \ldots &           B \\
 6392.54 &   26.0 &   2.28 & $-$3.97 &     50.1 &   \ldots &   \ldots &   \ldots &     65.4 &           B \\
 6481.88 &   26.0 &   2.28 & $-$2.98 &    101.7 &     94.5 &   \ldots &    103.7 &    121.4 &           B \\
 6498.94 &   26.0 &   0.96 & $-$4.70 &   \ldots &     92.7 &     86.3 &    104.7 &   \ldots &           B \\
 6518.37 &   26.0 &   2.83 & $-$2.46 &   \ldots &     77.2 &   \ldots &     81.9 &     99.8 &           B \\
 6533.94 &   26.0 &   4.56 & $-$1.29 &     51.8 &     42.4 &   \ldots &     50.9 &   \ldots &           B \\
 6593.88 &   26.0 &   2.43 & $-$2.42 &    116.8 &    110.7 &    115.2 &   \ldots &   \ldots &           B \\
 6608.04 &   26.0 &   2.28 & $-$3.96 &     50.5 &     44.9 &     35.3 &     48.8 &     69.5 &           B \\
 6627.56 &   26.0 &   4.55 & $-$1.50 &   \ldots &     35.5 &     30.3 &     40.8 &     60.0 &           B \\
 6648.08 &   26.0 &   1.01 & $-$5.92 &   \ldots &   \ldots &     27.9 &   \ldots &   \ldots &           C \\
 6699.16 &   26.0 &   4.59 & $-$2.17 &     18.4 &     12.7 &      9.2 &     15.0 &     25.5 &           C \\
 6703.58 &   26.0 &   2.76 & $-$3.01 &     67.0 &     58.2 &     57.3 &     68.9 &     85.2 &           B \\
 6713.75 &   26.0 &   4.80 & $-$1.41 &     30.9 &     24.2 &     21.6 &     24.6 &     45.1 &           B \\
 6725.36 &   26.0 &   4.10 & $-$2.21 &     29.6 &     29.2 &   \ldots &     26.9 &     44.9 &           B \\
 6726.67 &   26.0 &   4.61 & $-$1.10 &     57.1 &     51.2 &     54.4 &     54.2 &     73.4 &           B \\
 6733.15 &   26.0 &   4.64 & $-$1.44 &     39.4 &     29.8 &     27.8 &     39.0 &     54.0 &           B \\
 6739.52 &   26.0 &   1.56 & $-$4.82 &     41.6 &     39.9 &     30.4 &     45.4 &     64.2 &           C \\
 6750.16 &   26.0 &   2.42 & $-$2.62 &    105.2 &    100.3 &     99.2 &    113.8 &   \ldots &           B \\
 6786.86 &   26.0 &   4.19 & $-$1.90 &   \ldots &     34.2 &     29.9 &     41.6 &     54.8 &           B \\
 6806.86 &   26.0 &   2.73 & $-$3.14 &   \ldots &     58.5 &     55.9 &     68.5 &     83.5 &           B \\
 6810.27 &   26.0 &   4.61 & $-$1.01 &     60.8 &     55.0 &   \ldots &   \ldots &   \ldots &           B \\
 6820.37 &   26.0 &   4.64 & $-$1.17 &     55.6 &     46.5 &     43.1 &     53.9 &     73.0 &           B \\
 6839.83 &   26.0 &   2.56 & $-$3.35 &   \ldots &     60.1 &     55.8 &     69.0 &   \ldots &           B \\
 6843.66 &   26.0 &   4.55 & $-$0.85 &     75.0 &     63.8 &     63.2 &     75.3 &     90.1 &           B \\
 6855.72 &   26.0 &   4.61 & $-$1.71 &     36.5 &     30.8 &   \ldots &   \ldots &   \ldots &           B \\
 6857.25 &   26.0 &   4.08 & $-$2.07 &     38.2 &     30.9 &     25.9 &     34.2 &     51.1 &           B \\
 6858.16 &   26.0 &   4.61 & $-$0.95 &     60.1 &     54.1 &     51.5 &     65.8 &     76.5 &           B \\
 6861.94 &   26.0 &   2.42 & $-$3.78 &   \ldots &     43.3 &   \ldots &   \ldots &   \ldots &           B \\
 6971.93 &   26.0 &   3.02 & $-$3.39 &     33.5 &   \ldots &   \ldots &   \ldots &     52.1 &           C \\
 7112.17 &   26.0 &   2.99 & $-$3.04 &     65.3 &     52.8 &     48.7 &   \ldots &   \ldots &           C \\
 7189.15 &   26.0 &   3.07 & $-$2.83 &   \ldots &   \ldots &   \ldots &   \ldots &     81.2 &           C \\
 7223.66 &   26.0 &   3.02 & $-$2.27 &     94.5 &   \ldots &     82.7 &   \ldots &    110.7 &           C \\
 7401.69 &   26.0 &   4.18 & $-$1.66 &     59.7 &     49.7 &     45.6 &     53.5 &   \ldots &           C \\
 7710.36 &   26.0 &   4.22 & $-$1.13 &   \ldots &   \ldots &   \ldots &     80.0 &   \ldots &           C \\
 5197.58 &   26.1 &   3.23 & $-$2.23 &   \ldots &   \ldots &     86.5 &     84.4 &   \ldots &           B \\
 5234.63 &   26.1 &   3.22 & $-$2.22 &     75.3 &     75.7 &     89.7 &     87.0 &     84.5 &           B \\
 5264.81 &   26.1 &   3.34 & $-$3.21 &     42.0 &     44.0 &     50.6 &     51.0 &     47.0 &           B \\
 5325.56 &   26.1 &   3.22 & $-$3.18 &     36.8 &   \ldots &   \ldots &     46.9 &   \ldots &           B \\
 5425.26 &   26.1 &   3.20 & $-$3.27 &     40.6 &     36.7 &     43.8 &     45.8 &     45.1 &           B \\
 5991.38 &   26.1 &   3.15 & $-$3.56 &   \ldots &     30.6 &     37.5 &     39.8 &   \ldots &           B \\
 6149.25 &   26.1 &   3.89 & $-$2.73 &     32.6 &     30.3 &     38.2 &     37.2 &   \ldots &           B \\
 6247.56 &   26.1 &   3.89 & $-$2.33 &     42.3 &     44.8 &     51.3 &     54.2 &   \ldots &           B \\
 6369.46 &   26.1 &   2.89 & $-$4.21 &     18.2 &   \ldots &   \ldots &     21.4 &     22.4 &           B \\
 6416.93 &   26.1 &   3.89 & $-$2.70 &     37.2 &     34.7 &   \ldots &     44.0 &   \ldots &           B \\
 6432.68 &   26.1 &   2.89 & $-$3.58 &     42.8 &     40.4 &     46.4 &     50.3 &     43.0 &           B \\
 6516.08 &   26.1 &   2.89 & $-$3.38 &   \ldots &     53.5 &   \ldots &   \ldots &   \ldots &           B \\
 7711.72 &   26.1 &   3.90 & $-$2.54 &     40.2 &     36.2 &   \ldots &     46.9 &     48.3 &           C \\
 5003.75 &   28.0 &   1.68 & $-$3.13 &   \ldots &   \ldots &   \ldots &     73.2 &   \ldots &           B \\
 5010.94 &   28.0 &   3.64 & $-$0.90 &     54.6 &   \ldots &     57.4 &     60.2 &   \ldots &           B \\
 5048.85 &   28.0 &   3.85 & $-$0.37 &   \ldots &   \ldots &     83.9 &   \ldots &   \ldots &           B \\
 5094.42 &   28.0 &   3.83 & $-$1.12 &   \ldots &   \ldots &   \ldots &   \ldots &     48.2 &           B \\
 5157.98 &   28.0 &   3.61 & $-$1.72 &   \ldots &   \ldots &     21.1 &     27.8 &   \ldots &           B \\
 5197.17 &   28.0 &   3.90 & $-$1.14 &   \ldots &   \ldots &     28.2 &   \ldots &   \ldots &           B \\
 5578.73 &   28.0 &   1.68 & $-$2.67 &     90.0 &     88.0 &   \ldots &   \ldots &   \ldots &           B \\
 5587.87 &   28.0 &   1.94 & $-$2.37 &   \ldots &     83.0 &   \ldots &     89.0 &   \ldots &           B \\
 5589.37 &   28.0 &   3.90 & $-$1.15 &     40.5 &     33.6 &     30.6 &     37.8 &     50.2 &           B \\
 5593.75 &   28.0 &   3.90 & $-$0.79 &     54.2 &     50.9 &     46.3 &     54.3 &     66.5 &           B \\
 5643.09 &   28.0 &   4.17 & $-$1.25 &     24.5 &     21.6 &     17.2 &     26.9 &     35.0 &           B \\
 5748.36 &   28.0 &   1.68 & $-$3.25 &     65.5 &   \ldots &     58.0 &   \ldots &   \ldots &           B \\
 5805.23 &   28.0 &   4.17 & $-$0.60 &     54.4 &     45.1 &     43.2 &     52.8 &     64.7 &           B \\
 5847.01 &   28.0 &   1.68 & $-$3.44 &     64.5 &     57.2 &     49.2 &     62.3 &     79.7 &           B \\
 5996.74 &   28.0 &   4.24 & $-$1.06 &     35.1 &     26.2 &   \ldots &   \ldots &     45.1 &           B \\
 6007.31 &   28.0 &   1.68 & $-$3.34 &     55.5 &     55.5 &   \ldots &     61.7 &     73.2 &           A \\
 6053.69 &   28.0 &   4.24 & $-$1.07 &   \ldots &   \ldots &     23.8 &   \ldots &   \ldots &           B \\
 6108.12 &   28.0 &   1.68 & $-$2.49 &    102.5 &   \ldots &     94.2 &    105.4 &    118.3 &           B \\
 6111.08 &   28.0 &   4.09 & $-$0.83 &     54.3 &     43.4 &   \ldots &     49.1 &     60.4 &           B \\
 6128.98 &   28.0 &   1.68 & $-$3.39 &     61.1 &     57.9 &     52.4 &     68.3 &     79.2 &           B \\
 6130.14 &   28.0 &   4.27 & $-$0.98 &     33.8 &     29.1 &     22.5 &     34.0 &   \ldots &           B \\
 6175.37 &   28.0 &   4.09 & $-$0.53 &     61.4 &     53.8 &     50.0 &     62.9 &     69.3 &           A \\
 6176.82 &   28.0 &   4.09 & $-$0.26 &     75.9 &     67.2 &     65.8 &     76.2 &     90.3 &           B \\
 6177.25 &   28.0 &   1.83 & $-$3.60 &     46.2 &     38.4 &     34.1 &     44.4 &     57.2 &           B \\
 6186.72 &   28.0 &   4.11 & $-$0.90 &     45.4 &   \ldots &   \ldots &     42.8 &     58.6 &           B \\
 6204.61 &   28.0 &   4.09 & $-$1.15 &     37.8 &   \ldots &   \ldots &   \ldots &   \ldots &           B \\
 6223.99 &   28.0 &   4.11 & $-$0.97 &   \ldots &   \ldots &   \ldots &     42.7 &   \ldots &           B \\
 6322.17 &   28.0 &   4.15 & $-$1.21 &   \ldots &   \ldots &   \ldots &     29.8 &     40.6 &           B \\
 6378.26 &   28.0 &   4.15 & $-$0.82 &     46.4 &   \ldots &   \ldots &   \ldots &   \ldots &           B \\
 6482.81 &   28.0 &   1.94 & $-$2.85 &     80.5 &     73.7 &     72.0 &     85.5 &    108.6 &           B \\
 6532.88 &   28.0 &   1.94 & $-$3.42 &   \ldots &     40.5 &     37.4 &     47.6 &   \ldots &           B \\
 6586.32 &   28.0 &   1.95 & $-$2.79 &     80.8 &     73.9 &     69.2 &     86.2 &     97.0 &           B \\
 6767.78 &   28.0 &   1.83 & $-$2.11 &    111.3 &   \ldots &   \ldots &   \ldots &   \ldots &           B \\
 6772.32 &   28.0 &   3.66 & $-$1.01 &   \ldots &   \ldots &   \ldots &   \ldots &     77.3 &           B \\
 6842.04 &   28.0 &   3.66 & $-$1.44 &   \ldots &     39.2 &   \ldots &   \ldots &   \ldots &           B \\
 5105.50 &   29.0 &   1.39 & $-$1.50 &   \multicolumn{5}{c}{Spectrum synthesis}             &           D \\
 5782.14 &   29.0 &   1.39 & $-$1.70 &   \multicolumn{5}{c}{Spectrum synthesis}             &           D \\
 5853.69 &   56.1 &   0.60 & $-$0.91 &   \multicolumn{5}{c}{Spectrum synthesis}             &           E \\
 6141.73 &   56.1 &   0.70 & $-$0.03 &   \multicolumn{5}{c}{Spectrum synthesis}             &           E \\ 
 6496.91 &   56.1 &   0.60 & $-$0.41 &   \multicolumn{5}{c}{Spectrum synthesis}             &           E \\ 
 5290.84 &   57.1 &   0.00 & $-$1.65 &   \multicolumn{5}{c}{Spectrum synthesis}             &           F \\
 6262.29 &   57.1 &   0.43 & $-$1.22 &   \multicolumn{5}{c}{Spectrum synthesis}             &           F \\
 6645.13 &   63.1 &   1.37 &    0.12 &   \multicolumn{5}{c}{Spectrum synthesis}             &           G \\
\hline
\end{tabular}
\end{minipage}
\end{table*}



==> tab6.tex <==
\begin{table}
 \centering
 \begin{minipage}{80mm}
  \caption{Abundance errors from uncertainties in atmospheric parameters.}
  \label{tab:err} 
  \begin{tabular}{@{}lrrrrc@{}}
  \hline
        Species & 
        $\Delta$\teff & 
        $\Delta$\logg & 
        $\Delta$\vt & 
        $\Delta$[m/H] & 
        Total\footnote{The total error is determined by adding in quadrature
the first four entries. 
\\
This table is published in its entirety in the electronic edition of the paper.
A portion is shown here for guidance regarding its form and content.} \\
        & 
        +50 K  &
        +0.05 cgs &
        +0.2 \kms &
        +0.2 dex \\ 
\hline 
  \hline
\multicolumn{6}{c}{KIC 4350501} \\ 
$\Delta$[\oi/Fe]    & $-$0.10 &    0.04 &    0.06 & $-$0.04 &    0.13 \\
$\Delta$[\sii/Fe]   & $-$0.03 &    0.01 &    0.04 & $-$0.00 &    0.05 \\
$\Delta$[\cai/Fe]   &    0.05 & $-$0.01 & $-$0.01 & $-$0.01 &    0.05 \\
$\Delta$[\tii/Fe]   &    0.06 & $-$0.01 &    0.02 & $-$0.01 &    0.06 \\
$\Delta$[\cri/Fe]   &    0.04 & $-$0.01 &    0.01 & $-$0.01 &    0.04 \\
$\Delta$[\fei/H]    &    0.01 &    0.01 & $-$0.07 &    0.02 &    0.07 \\
$\Delta$[\feii/H]   & $-$0.07 &    0.04 & $-$0.06 &    0.02 &    0.10 \\
$\Delta$[\nii/Fe]   & $-$0.00 &    0.01 & $-$0.01 &    0.00 &    0.01 \\
$\Delta$[\cui/Fe]   &    0.03 & $-$0.01 & $-$0.00 &    0.04 &    0.05 \\
$\Delta$[\baii/Fe]  &    0.01 & $-$0.01 & $-$0.04 &    0.03 &    0.05 \\
$\Delta$[\laii/Fe]  &    0.01 &    0.01 &    0.03 &    0.01 &    0.03 \\
$\Delta$[\euii/Fe]  & $-$0.00 &    0.02 &    0.04 &    0.01 &    0.04 \\
\multicolumn{6}{c}{KIC 9821622} \\ 
$\Delta$[\oi/Fe]    & $-$0.08 &    0.02 &    0.05 &    0.02 &    0.10 \\
$\Delta$[\sii/Fe]   & $-$0.04 & $-$0.01 &    0.03 & $-$0.00 &    0.05 \\
$\Delta$[\cai/Fe]   &    0.03 & $-$0.01 & $-$0.03 & $-$0.01 &    0.04 \\
$\Delta$[\tii/Fe]   &    0.04 & $-$0.02 & $-$0.01 & $-$0.02 &    0.05 \\
$\Delta$[\cri/Fe]   &    0.02 & $-$0.01 &    0.01 & $-$0.01 &    0.03 \\
$\Delta$[\fei/H]    &    0.03 &    0.01 & $-$0.06 &    0.01 &    0.07 \\
$\Delta$[\feii/H]   & $-$0.05 &    0.02 & $-$0.06 &    0.03 &    0.09 \\
$\Delta$[\nii/Fe]   & $-$0.00 & $-$0.00 &    0.00 &    0.01 &    0.01 \\
$\Delta$[\cui/Fe]   &    0.02 & $-$0.01 & $-$0.03 &    0.03 &    0.05 \\
$\Delta$[\baii/Fe]  & $-$0.02 & $-$0.00 & $-$0.12 &    0.03 &    0.13 \\
$\Delta$[\laii/Fe]  & $-$0.01 &    0.01 &    0.03 &    0.03 &    0.04 \\
$\Delta$[\euii/Fe]  & $-$0.02 &    0.02 &    0.04 &    0.03 &    0.06 \\
\multicolumn{6}{c}{KIC 11394905} \\ 
$\Delta$[\oi/Fe]    & $-$0.07 &    0.04 &    0.05 &    0.04 &    0.10 \\
$\Delta$[\sii/Fe]   & $-$0.03 &    0.01 &    0.03 &    0.02 &    0.05 \\
$\Delta$[\cai/Fe]   &    0.02 & $-$0.00 & $-$0.02 & $-$0.00 &    0.03 \\
$\Delta$[\tii/Fe]   &    0.04 & $-$0.00 &    0.01 & $-$0.01 &    0.04 \\
$\Delta$[\cri/Fe]   &    0.02 & $-$0.00 &    0.00 & $-$0.00 &    0.02 \\
$\Delta$[\fei/H]    &    0.03 &    0.00 & $-$0.06 &    0.00 &    0.07 \\
$\Delta$[\feii/H]   & $-$0.05 &    0.04 & $-$0.06 &    0.04 &    0.10 \\
$\Delta$[\nii/Fe]   &    0.01 &    0.01 &    0.02 &    0.01 &    0.02 \\
$\Delta$[\cui/Fe]   &    0.02 & $-$0.00 & $-$0.10 &    0.02 &    0.10 \\
$\Delta$[\baii/Fe]  & $-$0.01 &    0.02 & $-$0.11 &    0.05 &    0.12 \\
$\Delta$[\laii/Fe]  & $-$0.02 &    0.02 &    0.03 &    0.04 &    0.06 \\
$\Delta$[\euii/Fe]  & $-$0.03 &    0.03 &    0.04 &    0.04 &    0.07 \\
\multicolumn{6}{c}{KIC 4143460} \\ 
$\Delta$[\oi/Fe]    & $-$0.07 &    0.03 &    0.05 & $-$0.01 &    0.09 \\
$\Delta$[\sii/Fe]   & $-$0.03 &    0.01 &    0.03 & $-$0.00 &    0.04 \\
$\Delta$[\cai/Fe]   &    0.03 & $-$0.02 & $-$0.04 & $-$0.02 &    0.06 \\
$\Delta$[\tii/Fe]   &    0.06 & $-$0.01 &    0.02 & $-$0.02 &    0.07 \\
$\Delta$[\cri/Fe]   &    0.04 & $-$0.00 &    0.01 & $-$0.01 &    0.04 \\
$\Delta$[\fei/H]    &    0.02 &    0.01 & $-$0.07 &    0.02 &    0.08 \\
$\Delta$[\feii/H]   & $-$0.05 &    0.05 & $-$0.06 &    0.03 &    0.10 \\
$\Delta$[\nii/Fe]   &    0.01 &    0.01 &    0.01 & $-$0.00 &    0.01 \\
$\Delta$[\cui/Fe]   &    0.03 & $-$0.01 & $-$0.04 &    0.02 &    0.06 \\
$\Delta$[\baii/Fe]  & $-$0.00 &    0.01 & $-$0.10 &    0.03 &    0.11 \\
$\Delta$[\laii/Fe]  & $-$0.00 &    0.02 &    0.04 &    0.02 &    0.05 \\
$\Delta$[\euii/Fe]  & $-$0.02 &    0.01 &    0.04 &    0.01 &    0.05 \\
\multicolumn{6}{c}{HD 40409} \\ 
$\Delta$[\oi/Fe]    & $-$0.05 &    0.01 &    0.07 &    0.02 &    0.09 \\
$\Delta$[\sii/Fe]   & $-$0.02 & $-$0.00 &    0.05 &    0.01 &    0.05 \\
$\Delta$[\cai/Fe]   &    0.05 & $-$0.02 & $-$0.00 & $-$0.02 &    0.06 \\
$\Delta$[\tii/Fe]   &    0.07 & $-$0.01 &    0.02 & $-$0.02 &    0.07 \\
$\Delta$[\cri/Fe]   &    0.05 & $-$0.01 & $-$0.00 & $-$0.01 &    0.05 \\
$\Delta$[\fei/H]    &    0.00 &    0.01 & $-$0.08 &    0.02 &    0.08 \\
$\Delta$[\feii/H]   & $-$0.06 &    0.03 & $-$0.06 &    0.05 &    0.10 \\
$\Delta$[\nii/Fe]   &    0.01 & $-$0.00 & $-$0.01 &    0.01 &    0.02 \\
$\Delta$[\cui/Fe]   &    0.03 & $-$0.01 & $-$0.00 &    0.03 &    0.04 \\
$\Delta$[\baii/Fe]  &    0.01 & $-$0.01 & $-$0.06 &    0.03 &    0.07 \\
$\Delta$[\laii/Fe]  &    0.02 &    0.01 &    0.04 &    0.02 &    0.05 \\
$\Delta$[\euii/Fe]  &    0.01 &    0.01 &    0.06 &    0.02 &    0.06 \\
  \hline
\end{tabular}
\end{minipage}
\end{table}


